Cell-Free Massive MIMO in the O-RAN Architecture: Cluster and Handover Strategies

Cell-free Massive MIMO has emerged as a promising solution for next-generation radio networks. Particularly the user-centric variant where users are served by a limited subset of access points, a so-called cluster, has garnered significant attention within the research community. Despite numerous proposed physical layer solutions, managing AP clusters in case of user mobility remains challenging. In this study, we first present a realistic method for modeling the temporal evolution of the channel in cell-free Massive MIMO. Next, we develop two clustering and handover strategies: 1) a fixed clustering strategy that computes the ideal cluster when a cluster handover threshold is exceeded and 2) an opportunistic strategy that opportunistically adds serving APs as the user moves. Moreover, we establish a connection between our findings and O-RAN, an emerging network architecture that offers open interfaces and network-wide control capabilities, thus, facilitating practical implementation of our research.

==> plots/fixedClusterSEs.tex <==
% \begin{figure}
% \centering
% \begin{subfigure}{0.5\linewidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%           width=0.8\linewidth, % Scale the plot to \linewidth
%           grid=major, % Display a grid
%           grid style={dashed,gray!30}, % Set the style
%           ylabel=CDF, % Set the labels
%           xlabel={SE [bits/s/Hz]},
%           xmin=0.0,
%           xmax= 4,
%           ymin=0,
%           ymax=1, 
% ytick={0, 0.25, 0.5, 0.75, 1},        
%           mark repeat=100,
%           legend columns=3,
%           %y unit=\si{\ampere},
%           legend style={at={(0.5,-0.3)},anchor=north}, % Put the legend below the plot
%                     legend style={nodes={scale=0.7, transform shape}},
%           x tick label style={rotate=0,anchor=north} % Display labels sideways
%         ]
%         \addplot table[x=1, y=CDF, col sep=comma,mark repeat=10] {figures/resultsFinal/UECentricCDF1.csv}; 
%         \addlegendentry{1 dB}
%         \addplot  table[x=2, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF1.csv};
%         \addlegendentry{2 dB}

%         \addplot  table[x=3, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF1.csv};
%         \addlegendentry{3 dB}

%         \addplot table[x=4, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF1.csv};
%         \addlegendentry{4 dB}
%         \addplot table[x=upper, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF1.csv};
%         \addlegendentry{Ubiquitous}
        
%         \addplot table[x=lower, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF1.csv};
        
%         \addlegendentry{Cellular}
        
%       \end{axis}
%     \end{tikzpicture}
%     % \caption{UE travelling at 30 km/h}
%      % \adam{Is the "O-RUs serving a user" the same as the serving cluster size?}}\robbert{yes}
% \end{subfigure}%
% \begin{subfigure}{0.5\linewidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%           width=0.8\linewidth, % Scale the plot to \linewidth
%           grid=major, % Display a grid
%           grid style={dashed,gray!30}, % Set the style
%           ylabel=CDF, % Set the labels
%           xlabel={SE [bits/s/Hz]},
%           xmin=0.0,
%           xmax= 4,
%           ymin=0,
%           ymax=1, 
% ytick={0, 0.25, 0.5, 0.75, 1},        
% mark repeat=100,
%           legend columns=3,
%           %y unit=\si{\ampere},
%           legend style={at={(0.5,-0.3)},anchor=north}, % Put the legend below the plot
%                     legend style={nodes={scale=0.7, transform shape}},
%           x tick label style={rotate=0,anchor=north} % Display labels sideways
%         ]
%         \addplot table[x=1, y=CDF, col sep=comma,mark repeat=10] {figures/resultsFinal/UECentricCDF2.csv}; 
%         \addlegendentry{1 dB}
%         \addplot  table[x=2, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF2.csv};
%         \addlegendentry{2 dB}
%         \addplot  table[x=3, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF2.csv};
%         \addlegendentry{3 dB}
%         \addplot table[x=4, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF2.csv};
%         \addlegendentry{4 dB}
%         \addplot table[x=upper, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF2.csv};
%         \addlegendentry{Ubiquitous}
%         \addplot table[x=lower, y=CDF, col sep=comma] {figures/resultsFinal/UECentricCDF2.csv};
%         \addlegendentry{Cellular}
%       \end{axis}
%     \end{tikzpicture}
%     % \caption{UE travelling at 120 km/h}
% \end{subfigure}
% \caption{Spectral Efficiency Distributions for UEs travelling at 30 km/h (left) and 120 km/h (right) for different HO thresholds for the fixed clustering and handover 
% strategy}   \label{fig:results1}
% \end{figure}

==> plots/opportunisticClusterSEs.tex <==
% \begin{figure}
% \begin{subfigure}{0.5\linewidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%           width=0.8\linewidth, % Scale the plot to \linewidth
%           grid=major, % Display a grid
%           grid style={dashed,gray!30}, % Set the style
%           ylabel=CDF, % Set the labels
%           xlabel={SE [bits/s/Hz]},
%           xmin=0.0,
%           xmax= 4,
%           ymin=0,
%           ymax=1, 
%           mark repeat=100,
% ytick={0, 0.25, 0.5, 0.75, 1},          
% legend columns=3,
%           %y unit=\si{\ampere},
%           legend style={at={(0.5,-0.3)},anchor=north}, % Put the legend below the plot
%           legend style={nodes={scale=0.7, transform shape}},
%           x tick label style={rotate=0,anchor=north} % Display labels sideways
%         ]
%         \addplot table[x=1, y=CDF, col sep=comma,mark repeat=10] {figures/resultsFinal/APCentricCDF1.csv}; 
%         \addlegendentry{1 dB}
%         \addplot  table[x=2, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF1.csv};
%         \addlegendentry{2 dB}

%         \addplot  table[x=3, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF1.csv};
%         \addlegendentry{3 dB}

%         \addplot table[x=4, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF1.csv};
%         \addlegendentry{4 dB}
        
%         \addplot table[x=upper, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF1.csv};
%         \addlegendentry{Ubiquitous}
        
%         \addplot table[x=lower, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF1.csv};
        
%         \addlegendentry{Cellular}
%       \end{axis}
%     \end{tikzpicture}
%     % \caption{30 km/h}
% \end{subfigure}%
% \begin{subfigure}{0.5\linewidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%           width=0.8\linewidth, % Scale the plot to \linewidth
%           grid=major, % Display a grid
%           grid style={dashed,gray!30}, % Set the style
%           ylabel=CDF, % Set the labels
%           xlabel={SE [bits/s/Hz]},
%           xmin=0.0,
%           xmax= 4,
%           ymin=0,
%           ytick={0, 0.25, 0.5, 0.75, 1},
%           ymax=1, 
%           mark repeat=100,
%           legend columns=3,
%           %y unit=\si{\ampere},
%          legend style={nodes={scale=0.7, transform shape}},
%           legend style={at={(0.5,-0.3)},anchor=north}, % Put the legend below the plot
%           x tick label style={rotate=0,anchor=north} % Display labels sideways
%         ]
%         \addplot table[x=1, y=CDF, col sep=comma,mark repeat=10] {figures/resultsFinal/APCentricCDF2.csv}; 
%         \addlegendentry{1 dB}
%         \addplot  table[x=2, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF2.csv};
%         \addlegendentry{2 dB}

%         \addplot  table[x=3, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF2.csv};
%         \addlegendentry{3 dB}

%         \addplot table[x=4, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF2.csv};
%         \addlegendentry{4 dB}8
        
%         \addplot table[x=upper, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF2.csv};
%         \addlegendentry{Ubiquitous}
        
%         \addplot table[x=lower, y=CDF, col sep=comma] {figures/resultsFinal/APCentricCDF2.csv};
        
%         \addlegendentry{Cellular}
%       \end{axis}
%     \end{tikzpicture}
%     % \caption{120 km/h}
% \end{subfigure}
% \caption{Spectral Efficiency Distributions for UEs travelling at 30 km/h (left) and 120 km/h (right) 
% for different HO thresholds for the opportunistic clustering and handover strategy.} 
% \label{fig:results2}
% \end{figure}

==> plots/systemmodelplots.tex <==
% \begin{figure}[htb]
% \centering
% \begin{subfigure}[t]{0.5\linewidth}
% \centering
% \begin{tikzpicture}
% \begin{axis}[ybar,
%         width=0.8\linewidth,
%             grid=major, % Display a grid
%           grid style={dashed,gray!30}, % Set the style
%         ymin=0,
%         ymax=1,  
%         % ymode=log,
%         % xtick = data
%         ylabel={Handover Frequency [$s^{-1}$]},
%         xlabel={UE Speed [km/h]},
%         xtick = {1,2,3,4},
%         % ytick = {3, 10, 30},
%         xticklabels = {
%             3,
%             30,
%             60,
%             120,
%         },
%         bar width=6pt,
%         x tick label style={rotate=0,anchor=north}, % Display labels sideways
%         xtick align=inside,
%         enlarge x limits=0.15,
%         % minor x tick num = 1,
%         % minor tick length=2ex,
%         legend pos = north west,
%         legend style={nodes={scale=0.6, transform shape}},
%         ]
%         \addplot[fill=blue]  table[x=deCorrDistance, y=1, col sep=comma] {figures/resultsChannelModel/CellularHandover.csv}; %
%                 \addlegendentry{20m}
%     \addplot[fill=red]  table[x=deCorrDistance,y=2, col sep=comma] {figures/resultsChannelModel/CellularHandover.csv};
%             \addlegendentry{50m}
%     \addplot[fill=brown]  table[x=deCorrDistance,y=3, col sep=comma]  {figures/resultsChannelModel/CellularHandover.csv};
%             \addlegendentry{100m}
%         \addplot[fill=black]  table[x=deCorrDistance,y=4, col sep=comma]  {figures/resultsChannelModel/CellularHandover.csv};
%                 \addlegendentry{200m}
%         \end{axis}
% \end{tikzpicture}
% \label{fig:results3}
% \end{subfigure}
% \begin{comment}

% \begin{subfigure}[t]{.5\linewidth}
% \centering
%     \begin{tikzpicture}[spy using outlines={magnification=5, rectangle, size=2cm}]
%       \begin{axis}[
%           width=0.8\linewidth, % Scale the plot to \linewidth
%           grid=major, % Display a grid
%           grid style={dashed,gray!30}, % Set the style
%           ylabel=CDF, % Set the labels
%           xlabel={SE [bits/s/Hz]},
%           xmin=0.0,
%           xmax= 4,
%           ymin=0,
%           ymax=1, 
%           ytick={0, 0.25, 0.5, 0.75, 1},        
%           mark repeat=100,
%           legend columns=2,
%           %y unit=\si{\ampere},
%           legend pos = south east,
%                   legend style={nodes={scale=0.6, transform shape}},
%           x tick label style={rotate=0,anchor=north} % Display labels sideways
%         ]
%         \addplot table[x=1, y=cdf, col sep=comma,mark repeat=10] {figures/resultsChannelModel/CellularSEs.csv}; 
%         \addlegendentry{20 m}
%         \addplot  table[x=2, y=cdf, col sep=comma] {figures/resultsChannelModel/CellularSEs.csv}; 
%         \addlegendentry{50 m}

%         \addplot  table[x=3, y=cdf, col sep=comma] {figures/resultsChannelModel/CellularSEs.csv}; 
%         \addlegendentry{100 m}

%         \addplot table[x=4, y=cdf, col sep=comma] {figures/resultsChannelModel/CellularSEs.csv}; 
%         \addlegendentry{200 m}
%         \coordinate (spypoint) at (axis cs:1.25,0.52);
%       \end{axis}
%       % \spy on (spypoint) in node at (4.5, 2.5);
%     \end{tikzpicture}
%     \caption{Effect on the CDF of the SE}
%     \label{fig:results1}
% \end{subfigure}%
% \end{comment}
% \caption{Effect of the decorrelation distance $\frac{1}{\alpha}$ on the handover frequency of the cellular case for UEs travelling at various speeds}
% % \sofie{Why is there no impact on SE? Is your handover too perfect?  } \sofie{Which handover? opportunistic or fixed?}}\robbert{cellular case, handover 
% % and LSFD is calculated at the same time instances}%
% \label{fig:resdecorr}
% \end{figure}

==> symbols.tex <==
\begin{table}[htb]
\caption{List of symbols}

\centering
\begin{tabularx}{\textwidth}{l|X||l|X}

Symbol    & Definition & Symbol & Definition \\ \hline
$K$         & Total number of UEs       &    $C$    &  Number of O-DUs \\ \hline
$L$         & Total number of O-RUs         &   $N$     & Number of antennas per O-RU           \\ \hline

$\hat{\mathbf{h}}_{l,k}$ & Estimated channel vector between UE $k$ and O-RU $l$ & $\mathbf{h}_{l,k}$     & Channel Vector between UE $k$ and O-RU $l$            \\ \hline
$\beta_{l,k}[t]$        &  Channel Gain between UE $k$ and O-RU $l$ at time $t$      & $\beta_{l,k}^{\text{dB}}[t]$ & Channel gain between UE $k$ and O-RU $l$ at time $t$ expressed in dB   \\  \hline
$\mathcal{M}_k^{\text{s}}[t]$        &  Serving Cluster for UE $k$ at time $t$         &  $\mathcal{M}_k^{\text{m}}$       &     Measurement Cluster for UE $k$       \\ \hline
$O_k[t]$ & Function that selects best O-RUs from measurment cluster for UE $k$ at time $t$      &  $Q^{(w)}_l[t]$      &    Function that selects $w$ best UEs for O-RU $l$ at time $t$        \\ \hline
$l_k^{\ast}$ & Index of primary O-RU for UE $k$ &  $K^{\ast}_l$ & Number of UEs that use O-RU $l$ as primary O-RU \\ \hline
$\mathbf{a}_k$ & LSFD combiner for UE $k$ & $\mathbf{v}_{l, k}$ & Receive combiner for UE $k$ in O-RU $l$ \\ \hline 
 $\mathcal{D}_l$ & Set of UEs that are served by O-RU $l$ & $p_k$ & UL power of UE $k$ \\ \hline
$\mathbf{R}_{l,k}$ & Covariance matrix of channel between UE $k$ and O-RU $l$ &  $\mathbf{C}_{l,k}$ & Channel estimation error covariance matrix between UE $k$ and O-RU $l$\\ \hline
$\mathcal{P}_k$ & Set of UEs that share the pilot with UE $k$ & $\tau_p$ & Length of the pilot sequence \\\hline
$\phi_{t_k}$ & Pilot sequence with index $t_k$ & $\mathbf{n}_l$ & Received noise 
vector at O-RU $l$ \\ \hline 
$s_k$ & Symbol transmitted by UE $k$ & $\hat{s}_{l,k}$ & Estimate for received signal from UE $k$ at O-RU $l$ \\ \hline
$\mathbf{g}_{ki}$ & Effective gain for UE $i$ in the combining vector for UE $k$ & $F_{l,k}[t]$ & Shadow fading between UE $k$ and O-RU $l$ at time $t$ \\ 

\end{tabularx}
%\caption{List of symbols}
\label{table:symbols}
\end{table}
